Implicit Assimilation of Sparse In Situ Data for Dense & Global Storm Surge Forecasting

Hurricanes and coastal floods are among the most disastrous natural hazards. Both are intimately related to storm surges, as their causes and effects, respectively. However, the short-term forecasting of storm surges has proven challenging, especially when targeting previously unseen locations or sites without tidal gauges. Furthermore, recent work improved short and medium-term weather forecasting but the handling of raw unassimilated data remains non-trivial. In this paper, we tackle both challenges and demonstrate that neural networks can implicitly assimilate sparse in situ tide gauge data with coarse ocean state reanalysis in order to forecast storm surges. We curate a global dataset to learn and validate the dense prediction of storm surges, building on preceding efforts. Other than prior work limited to known gauges, our approach extends to ungauged sites, paving the way for global storm surge forecasting.

==> Fig/figure_1_backup.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,372); %set diagram left start at 0, and has height of 372

%Image [id:dp447919462677264] 
\draw (330.24,133.36) node  {\includegraphics[width=45.6pt,height=45.6pt]{Fig/bunch/3/utae/4_out_model_masked.png}};
%Image [id:dp8969336409330839] 
\draw (330.24,244.36) node  {\includegraphics[width=45.6pt,height=45.6pt]{Fig/bunch/3/coarse/4_out_model_masked.png}};
%Image [id:dp8806348634582146] 
\draw (89.84,83.76) node  {\includesvg[width=45.6pt,height=45.6pt]{Fig/bunch/3/4_in_scatter_lsm.svg}};
%Shape: Rectangle [id:dp5536973774369096] 
\draw   (59.44,53.36) -- (120.24,53.36) -- (120.24,114.16) -- (59.44,114.16) -- cycle ;

%Image [id:dp8377017738175867] 
\draw (79.84,93.76) node  {\includesvg[width=45.6pt,height=45.6pt]{Fig/bunch/3/4_in_scatter_lsm.svg}};
%Shape: Rectangle [id:dp664568679343208] 
\draw   (49.44,63.36) -- (110.24,63.36) -- (110.24,124.16) -- (49.44,124.16) -- cycle ;
%Image [id:dp991104573465732] 
\draw (89.84,283.6) node  {\includegraphics[width=45.6pt,height=45.6pt]{Fig/bunch/3/4_msl_era5_grey.png}};
%Shape: Rectangle [id:dp9168500499894487] 
\draw   (59.44,253.2) -- (120.24,253.2) -- (120.24,314) -- (59.44,314) -- cycle ;
%Image [id:dp2921782273796041] 
\draw (79.84,293.76) node  {\includegraphics[width=45.6pt,height=45.6pt]{Fig/bunch/3/4_msl_era5_grey.png}};
%Shape: Rectangle [id:dp14977439390228797] 
\draw   (49.44,263.36) -- (110.24,263.36) -- (110.24,324.16) -- (49.44,324.16) -- cycle ;
%Image [id:dp7614995495202921] 
\draw (89.84,183.76) node  {\includegraphics[width=45.6pt,height=45.6pt]{Fig/bunch/3/gtsm/4_out_model_masked.png}};
%Shape: Rectangle [id:dp04569238864000269] 
\draw   (59.44,153.36) -- (120.24,153.36) -- (120.24,214.16) -- (59.44,214.16) -- cycle ;
%Image [id:dp2794154968385454] 
\draw (79.84,193.76) node  {\includegraphics[width=45.6pt,height=45.6pt]{Fig/bunch/3/gtsm/4_out_model_masked.png}};


%Shape: Rectangle [id:dp5847485781911803] 
\draw   (49.44,163.36) -- (110.24,163.36) -- (110.24,224.16) -- (49.44,224.16) -- cycle ;
%Straight Lines [id:da2796424587449289] 
\draw    (115.04,337.6) -- (142.64,313.9) ;
\draw [shift={(144.16,312.6)}, rotate = 139.35] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Ellipse [id:dp7223231547149207] 
\draw  [fill={rgb, 255:red, 37; green, 37; blue, 37 }  ,fill opacity=0.5 ] (126.4,301.55) .. controls (126.4,300.53) and (127.27,299.7) .. (128.35,299.7) .. controls (129.42,299.7) and (130.3,300.53) .. (130.3,301.55) .. controls (130.3,302.57) and (129.42,303.4) .. (128.35,303.4) .. controls (127.27,303.4) and (126.4,302.57) .. (126.4,301.55) -- cycle ;
%Shape: Ellipse [id:dp8290124492611026] 
\draw  [fill={rgb, 255:red, 37; green, 37; blue, 37 }  ,fill opacity=0.5 ] (130.77,298) .. controls (130.77,296.98) and (131.64,296.15) .. (132.72,296.15) .. controls (133.8,296.15) and (134.67,296.98) .. (134.67,298) .. controls (134.67,299.02) and (133.8,299.84) .. (132.72,299.84) .. controls (131.64,299.84) and (130.77,299.02) .. (130.77,298) -- cycle ;
%Shape: Ellipse [id:dp6183168257340075] 
\draw  [fill={rgb, 255:red, 37; green, 37; blue, 37 }  ,fill opacity=0.5 ] (135.14,293.85) .. controls (135.14,292.83) and (136.02,292) .. (137.09,292) .. controls (138.17,292) and (139.04,292.83) .. (139.04,293.85) .. controls (139.04,294.87) and (138.17,295.7) .. (137.09,295.7) .. controls (136.02,295.7) and (135.14,294.87) .. (135.14,293.85) -- cycle ;
%Shape: Ellipse [id:dp3914168288159803] 
\draw  [fill={rgb, 255:red, 37; green, 37; blue, 37 }  ,fill opacity=0.5 ] (126.4,201.55) .. controls (126.4,200.53) and (127.27,199.7) .. (128.35,199.7) .. controls (129.42,199.7) and (130.3,200.53) .. (130.3,201.55) .. controls (130.3,202.57) and (129.42,203.4) .. (128.35,203.4) .. controls (127.27,203.4) and (126.4,202.57) .. (126.4,201.55) -- cycle ;
%Shape: Ellipse [id:dp060645764745941744] 
\draw  [fill={rgb, 255:red, 37; green, 37; blue, 37 }  ,fill opacity=0.5 ] (130.77,198) .. controls (130.77,196.98) and (131.64,196.15) .. (132.72,196.15) .. controls (133.8,196.15) and (134.67,196.98) .. (134.67,198) .. controls (134.67,199.02) and (133.8,199.84) .. (132.72,199.84) .. controls (131.64,199.84) and (130.77,199.02) .. (130.77,198) -- cycle ;
%Shape: Ellipse [id:dp8395546364347912] 
\draw  [fill={rgb, 255:red, 37; green, 37; blue, 37 }  ,fill opacity=0.5 ] (135.14,193.85) .. controls (135.14,192.83) and (136.02,192) .. (137.09,192) .. controls (138.17,192) and (139.04,192.83) .. (139.04,193.85) .. controls (139.04,194.87) and (138.17,195.7) .. (137.09,195.7) .. controls (136.02,195.7) and (135.14,194.87) .. (135.14,193.85) -- cycle ;
%Shape: Ellipse [id:dp8940361792527816] 
\draw  [fill={rgb, 255:red, 37; green, 37; blue, 37 }  ,fill opacity=0.5 ] (130.77,98) .. controls (130.77,96.98) and (131.64,96.15) .. (132.72,96.15) .. controls (133.8,96.15) and (134.67,96.98) .. (134.67,98) .. controls (134.67,99.02) and (133.8,99.84) .. (132.72,99.84) .. controls (131.64,99.84) and (130.77,99.02) .. (130.77,98) -- cycle ;
%Shape: Ellipse [id:dp7614592229575639] 
\draw  [fill={rgb, 255:red, 37; green, 37; blue, 37 }  ,fill opacity=0.5 ] (135.14,93.85) .. controls (135.14,92.83) and (136.02,92) .. (137.09,92) .. controls (138.17,92) and (139.04,92.83) .. (139.04,93.85) .. controls (139.04,94.87) and (138.17,95.7) .. (137.09,95.7) .. controls (136.02,95.7) and (135.14,94.87) .. (135.14,93.85) -- cycle ;
%Shape: Trapezoid [id:dp5814960922282624] 
\draw   (159.8,67.2) -- (211.04,87.16) -- (211.04,290.44) -- (159.8,310.4) -- cycle ;
%Shape: Rectangle [id:dp6401588549019526] 
\draw   (217.6,88.6) -- (236.96,88.6) -- (236.96,289.92) -- (217.6,289.92) -- cycle ;
%Shape: Rectangle [id:dp36063838643196244] 
\draw   (244.6,88.6) -- (263.64,88.6) -- (263.64,179.96) -- (244.6,179.96) -- cycle ;
%Shape: Rectangle [id:dp3907215794083556] 
\draw   (244.6,199.16) -- (263.64,199.16) -- (263.64,289.92) -- (244.6,289.92) -- cycle ;
%Shape: Rectangle [id:dp2877959525906373] 
\draw   (299.84,102.96) -- (360.64,102.96) -- (360.64,163.76) -- (299.84,163.76) -- cycle ;
%Shape: Rectangle [id:dp5846049496913888] 
\draw   (299.84,213.96) -- (360.64,213.96) -- (360.64,274.76) -- (299.84,274.76) -- cycle ;
%Shape: Ellipse [id:dp33947761463750714] 
\draw  [fill={rgb, 255:red, 37; green, 37; blue, 37 }  ,fill opacity=0.5 ] (80.4,247.55) .. controls (80.4,246.53) and (81.27,245.7) .. (82.35,245.7) .. controls (83.42,245.7) and (84.3,246.53) .. (84.3,247.55) .. controls (84.3,248.57) and (83.42,249.4) .. (82.35,249.4) .. controls (81.27,249.4) and (80.4,248.57) .. (80.4,247.55) -- cycle ;
%Shape: Ellipse [id:dp6147102621664717] 
\draw  [fill={rgb, 255:red, 37; green, 37; blue, 37 }  ,fill opacity=0.5 ] (87.4,247.55) .. controls (87.4,246.53) and (88.27,245.7) .. (89.35,245.7) .. controls (90.42,245.7) and (91.3,246.53) .. (91.3,247.55) .. controls (91.3,248.57) and (90.42,249.4) .. (89.35,249.4) .. controls (88.27,249.4) and (87.4,248.57) .. (87.4,247.55) -- cycle ;
%Shape: Ellipse [id:dp726103188473175] 
\draw  [fill={rgb, 255:red, 37; green, 37; blue, 37 }  ,fill opacity=0.5 ] (94.4,247.55) .. controls (94.4,246.53) and (95.27,245.7) .. (96.35,245.7) .. controls (97.42,245.7) and (98.3,246.53) .. (98.3,247.55) .. controls (98.3,248.57) and (97.42,249.4) .. (96.35,249.4) .. controls (95.27,249.4) and (94.4,248.57) .. (94.4,247.55) -- cycle ;
%Straight Lines [id:da5974645044936182] 
\draw [line width=1.5]    (127.4,84.8) -- (150.4,84.8) ;
\draw [shift={(153.4,84.8)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Straight Lines [id:da919971573337679] 
\draw [line width=1.5]    (127.4,185.8) -- (150.4,185.8) ;
\draw [shift={(153.4,185.8)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Straight Lines [id:da13647720449623568] 
\draw [line width=1.5]    (127.4,284.8) -- (150.4,284.8) ;
\draw [shift={(153.4,284.8)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Straight Lines [id:da6385629846948022] 
\draw [line width=1.5]    (266,134.92) -- (291.4,134.45) ;
\draw [shift={(294.4,134.4)}, rotate = 178.95] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Straight Lines [id:da5758057412452724] 
\draw [line width=1.5]    (266,244.92) -- (291.4,244.45) ;
\draw [shift={(294.4,244.4)}, rotate = 178.95] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Shape: Ellipse [id:dp68858258443389] 
\draw  [fill={rgb, 255:red, 37; green, 37; blue, 37 }  ,fill opacity=0.5 ] (125.77,102) .. controls (125.77,100.98) and (126.64,100.15) .. (127.72,100.15) .. controls (128.8,100.15) and (129.67,100.98) .. (129.67,102) .. controls (129.67,103.02) and (128.8,103.84) .. (127.72,103.84) .. controls (126.64,103.84) and (125.77,103.02) .. (125.77,102) -- cycle ;

% Text Node
\draw (116.04,339) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$1$};
% Text Node
\draw (125.84,331) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$2$};
% Text Node
\draw (168.6,255.92) node [anchor=north west][inner sep=0.75pt]  [rotate=-270] [align=left] {\begin{minipage}[lt]{95.15pt}\setlength\topsep{0pt}
\begin{center}
Spatio-temporal\\deep neural network
\end{center}

\end{minipage}};
% Text Node
\draw (218,270.32) node [anchor=north west][inner sep=0.75pt]  [rotate=-270] [align=left] {\begin{minipage}[lt]{119.52pt}\setlength\topsep{0pt}
\begin{center}
Spatial parameter sharing
\end{center}

\end{minipage}};
% Text Node
\draw (21.4,28.2) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{Input} sequence of length $T$};
% Text Node
\draw (251.76,28.28) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{Output} for lead time $\displaystyle L$};
% Text Node
\draw (312.64,282.8) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$( T+L)$};
% Text Node
\draw (9.2,125.92) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,rotate=-270] [align=left] {\begin{minipage}[lt]{52.62pt}\setlength\topsep{0pt}
\begin{center}
Sparse in-situ\\tide gages
\end{center}

\end{minipage}};
% Text Node
\draw (9,230.92) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,rotate=-270] [align=left] {\begin{minipage}[lt]{59.42pt}\setlength\topsep{0pt}
\begin{center}
Coarse ocean\\state reanalysis
\end{center}

\end{minipage}};
% Text Node
\draw (9,330.92) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,rotate=-270] [align=left] {\begin{minipage}[lt]{59.42pt}\setlength\topsep{0pt}
\begin{center}
Atmosphere\\state reanalysis
\end{center}

\end{minipage}};
% Text Node
\draw (363,172.92) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,rotate=-270] [align=left] {\begin{minipage}[lt]{59.41pt}\setlength\topsep{0pt}
\begin{center}
Densified storm\\surge forecast
\end{center}

\end{minipage}};
% Text Node
\draw (363,288.92) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,rotate=-270] [align=left] {\begin{minipage}[lt]{60.32pt}\setlength\topsep{0pt}
\begin{center}
Auxiliary coarse\\state forecast
\end{center}

\end{minipage}};
% Text Node
\draw (131.06,327.17) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,rotate=-316.28]  {$...$};
% Text Node
\draw (144.84,314) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$T$};


\end{tikzpicture}

